Linear Dynamics: Clustering without identification

Linear dynamical systems are a fundamental and powerful parametric model class. However, identifying the parameters of a linear dynamical system is a venerable task, permitting provably efficient solutions only in special cases. This work shows that the eigenspectrum of unknown linear dynamics can be identified without full system identification. We analyze a computationally efficient and provably convergent algorithm to estimate the eigenvalues of the state-transition matrix in a linear dynamical system. When applied to time series clustering, our algorithm can efficiently cluster multi-dimensional time series with temporal offsets and varying lengths, under the assumption that the time series are generated from linear dynamical systems. Evaluating our algorithm on both synthetic data and real electrocardiogram (ECG) signals, we see improvements in clustering quality over existing baselines.

==> comments.tex <==
\begin{document}
\section{Comments from Moritz}

Some comments from April 22, 2019:

\begin{itemize}
\item I was going to suggest using the \emph{controllable canonical form} for the linear system. But then I saw that you rederived it as the companion matrix. This is a known thing that exists when the eigenvalues of $A$ are distinct and should simplify the analysis in this case.
\item You can combine the analysis you have with estimation bounds for learning ARMA models. This will give you a method for learning linear dynamical systems. That opens up a lot of relevant literature. You found Max's paper, but there are a few more. Elad Hazan's group has been looking into this recently, e.g., \url{https://papers.nips.cc/paper/7714-spectral-filtering-for-general-linear-dynamical-systems.pdf}. You can also have a look at the paper I had with Tengyu and Ben. It's not super relevant, but I'm curious if the assumption we make in that paper simplifies things in our setting. It was immediately clear to me how and it's not a very natural assumption anyway. So, no need to dig too deep here.
\item A lot of the existing results for learning linear dynamical systems make use of overparameterization. In our setting, this would correspond to giving the ARMA model extra parameters compared with the target system. I'm curious to see how this plays out. It might require going about the analysis a bit differently, since you'd no longer recover the parameters.
\item Given the results, we have a bit of a decision to make: Will this be a paper on learning linear dynamical systems, or on clustering. We can wait with the final call on this, but it's worth keeping this in mind. My gut instict would be to stick with clustering unless the LDS component starts to become competitive with state-of-the-art for that problem.
\item I had a quick chat with Max Simchowitz about prior and related work. Max thinks that the model equivalence between ARMA and LDS is well known. However, I'm not so sure if people have explored exactly what assumptions lead to nice results. There may be assumptions that are natural from a learning perspective that people haven't explored. 
\item What's not settled is the estimation part for ARMA models. While AR models are easy, ARMA models not necessarily so, especially when they have inputs (ARMAX?). Apparently, people have used some recursive least squares for this. A recent paper to look at on this topic is this: \url{https://arxiv.org/abs/1903.09122}.
\item Another thought: The problem of clustering time series is at least as hard as mixture learning. You could always take a mixture of $k$ gaussians as generating your samples. Once you cluster the time series, you can then learn inside each cluster to get the parameters of the gaussian for that cluster. So whatever hardness results hold for mixtures of gaussians will also apply here. If you have a fixed dimensional model, the problem should get easier with longer sequences as you get more separation. But this is something to think about and perhaps spell out the reduction. In general, for example, we get the hardness of learning mixtures of $k$ gaussians, which will have the $1/k$ exponent in the estimation rate.
\end{itemize}


\section{Re: Comments from Moritz}

From Chloe, re: comments from April 22, 2019.

\begin{itemize}
\item I was going to suggest using the \emph{controllable canonical form} for the linear system. But then I saw that you rederived it as the companion matrix. This is a known thing that exists when the eigenvalues of $A$ are distinct and should simplify the analysis in this case.
\item[$\vartriangleright$] Thanks for pointing out this connection. It was really interesting to read about controllable canonical form in your paper with Tengyu and Ben. 

The bulk of the current analysis is to bound the condition number for eigenvalue of the controllable canonical form, i.e. how much the eigenvalue changes when the controllable canonical form changes. Upon a quick search haven't found any direct reference for this condition number, but I'm entirely new to control theory so I'll look around more.
\item You can combine the analysis you have with estimation bounds for learning ARMA models. This will give you a method for learning linear dynamical systems. That opens up a lot of relevant literature. You found Max's paper, but there are a few more. Elad Hazan's group has been looking into this recently, e.g., \url{https://papers.nips.cc/paper/7714-spectral-filtering-for-general-linear-dynamical-systems.pdf}. You can also have a look at the paper I had with Tengyu and Ben. It's not super relevant, but I'm curious if the assumption we make in that paper simplifies things in our setting. It was immediately clear to me how and it's not a very natural assumption anyway. So, no need to dig too deep here.
\item[$\vartriangleright$] I thought about that possibility a little bit, and it seems pretty challenging to be competitive with state-of-the-art. Compared to Elad's paper, their result do not depend on the spectrum of the LDS, and my sense is that the result from this method might have to depend on the spectrum. 

Regarding your paper with Tengyu and Ben, the autoregressive part of the ARMA model is in some sense just another way to express the controllable canonical form. The controllability and stability conditions are similar to the assumptions in equation (\ref{stable_condition_number_bound}) (with the difference of whether the spectral radius is \textit{strictly} bounded from 1). The unit circle cone condition might be applied to simplify the analysis of $\prod_{k \neq j} (\lambda_k - \lambda_j)$, when the roots are more dispersed.

One question in this direction: If we use an existing ARMA estimation method to learn the controllable canonical form instead of gradient descent, and then combine the estimation bound with the rest of the analysis in the paper, would this give us a tighter bound?

Another question in the inverse direction: Can we use the projected stochastic gradient descent method to estimate ARMA parameters better?

\item A lot of the existing results for learning linear dynamical systems make use of overparameterization. In our setting, this would correspond to giving the ARMA model extra parameters compared with the target system. I'm curious to see how this plays out. It might require going about the analysis a bit differently, since you'd no longer recover the parameters.

\item[$\vartriangleright$] Haven't thought much about over-parameterization. I'm also curious to find out. My initial impression was that in time series analysis people usually try to pick the exact right number of autoregressive steps, so maybe it would hurt to have extra parameters, but not sure if this will be what analysis says.

\item Given the results, we have a bit of a decision to make: Will this be a paper on learning linear dynamical systems, or on clustering. We can wait with the final call on this, but it's worth keeping this in mind. My gut instict would be to stick with clustering unless the LDS component starts to become competitive with state-of-the-art for that problem.
\item[$\vartriangleright$] Agreed to stick with clustering. I think there are interesting questions here related to learning dynamical systems, but maybe would be more suitable as separate future work.

Other than clustering, we could also try supervised classification, i.e. nearest neighbor classifier, depending on what labels are in the datasets.

\item I had a quick chat with Max Simchowitz about prior and related work. Max thinks that the model equivalence between ARMA and LDS is well known. However, I'm not so sure if people have explored exactly what assumptions lead to nice results. There may be assumptions that are natural from a learning perspective that people haven't explored. 
\item[$\vartriangleright$] Thanks for getting Max's expert perspective. That's helpful to know. When searching for prior work I struggled quite a bit with finding the right keywords - I wasn't able to find good reference on the exact correspondence between ARMA and LDS, but it wouldn't be surprising at all if this is well known, given that both ARMA and LDS are relatively well studied.

\item What's not settled is the estimation part for ARMA models. While AR models are easy, ARMA models not necessarily so, especially when they have inputs (ARMAX?). Apparently, people have used some recursive least squares for this. A recent paper to look at on this topic is this: \url{https://arxiv.org/abs/1903.09122}.
\item[$\vartriangleright$] Will read more about recursive least squares, and curious to see if analysis of ARMA parameter estimation will lead to the $1/k$ exponent in the estimation rate mentioned below.

\item Another thought: The problem of clustering time series is at least as hard as mixture learning. You could always take a mixture of $k$ gaussians as generating your samples. Once you cluster the time series, you can then learn inside each cluster to get the parameters of the gaussian for that cluster. So whatever hardness results hold for mixtures of gaussians will also apply here. If you have a fixed dimensional model, the problem should get easier with longer sequences as you get more separation. But this is something to think about and perhaps spell out the reduction. In general, for example, we get the hardness of learning mixtures of $k$ gaussians, which will have the $1/k$ exponent in the estimation rate.
\end{itemize}



\section*{Sample figure and table}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\end{document}

==> scratch.tex <==
\section{Additional ECG clustering results}

\begin{table}
\begin{tabular}{lllr}
\toprule
Label &  Meaning & Occurrence & Selected in~\cite{ozbay2006fuzzy} \\
\midrule
N & Normal sinus rhythm    &    529 & Y\\
B    &  Ventricular bigeminy & 221 & N\\
AFIB & Atrial fibrillation  & 107 & Y\\
PREX & Pre-excitation (WPW)  & 103 & N\\
T    &  Ventricular trigeminy &  83 & N\\
VT   &  Ventricular tachycardia &  61 & Y \\
P    &  Paced rhythm  & 60 & Y\\
AFL  &  Atrial flutter &  45 & Y\\
NOD  &  Nodal (A-V junctional) rhythm  & 36 & N \\
SVTA &  Supraventricular tachyarrhythmia &  26 & N\\
VFL  &  Ventricular flutter  &  6 & N\\
BII  &  2$^{\circ}$ heart block &   5 & N\\
IVR  &  Idioventricular rhythm  &  4 & N\\
AB & Atrial bigeminy   &      3 & N\\
SBR  &  Sinus bradycardia  &  1 & Y\\
\midrule
Total & & 1290 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{Label prevalence and label meanings in the MIT-BIH Arrhythmia Database. The types are selected according the experiment setup in~\cite{ozbay2006fuzzy}.}
\end{table}
